Can Visual Context Improve Automatic Speech Recognition for an Embodied Agent?

The usage of automatic speech recognition (ASR) systems are becoming omnipresent ranging from personal assistant to chatbots, home, and industrial automation systems, etc. Modern robots are also equipped with ASR capabilities for interacting with humans as speech is the most natural interaction modality. However, ASR in robots faces additional challenges as compared to a personal assistant. Being an embodied agent, a robot must recognize the physical entities around it and therefore reliably recognize the speech containing the description of such entities. However, current ASR systems are often unable to do so due to limitations in ASR training, such as generic datasets and open-vocabulary modeling. Also, adverse conditions during inference, such as noise, accented, and far-field speech makes the transcription inaccurate. In this work, we present a method to incorporate a robot's visual information into an ASR system and improve the recognition of a spoken utterance containing a visible entity. Specifically, we propose a new decoder biasing technique to incorporate the visual context while ensuring the ASR output does not degrade for incorrect context. We achieve a 59% relative reduction in WER from an unmodified ASR system.

==> related.tex <==
\section{Related work}
\label{sec:related}
There has been an increasing interest in contextual speech recognition, primarily applied to voice-based assistants~\citep{williams2018contextual,pundak2018deep,chen2019end,he2019streaming,gourav2021personalization,le2021contextualized}. However, incorporating visual context into a speech recognizer is usually modeled as a multi-modal speech recognition problem~\citep{michelsanti2021overview}, often simplified to lip-reading~\citep{ghorbani2021listen}. Initial attempts to utilize visual context in robotic agents also follow the same approach~\citep{ONEATA2021106943}. Such models always require a multi-modal (i.e., a pair of speech and visual) input, which fails to tackle cases where the visual context is irrelevant to the speech. 

In contrast, we consider the visual context as a source of dynamic prior knowledge. Thus, we bias the prediction of the speech recognizer to include information from the prior knowledge, provided some relevant information is found. There are two primary approaches to introducing bias in an ASR system, namely shallow and deep fusion. Shallow fusion based approaches perform re-scoring of transcription hypotheses upon detection of biasing words during beam search~\citep{williams2018contextual,kannan2018analysis}. Class-based language models have been proposed to utilize the prefix context of biasing words~\citep{chen2019end,kang2020fast}. \citep{zhao2019shallow} further improved the shallow-fusion biasing model by introducing bias at the sub-word boundaries and prefix-based activation of bias.~\citep{gourav2021personalization} proposed 2-pass re-scoring with a neural language model (LM), along with sub-word based biasing for more effective shallow-fusion. 

Deep-fusion biasing approaches use a pre-set biasing vocabulary to encode biasing phrases into embeddings that are applied using an attention-based decoder~\citep{pundak2018deep}. This is further improved by using adversarial examples~\citep{alon2019contextual}, complex attention-modeling~\citep{chang2021context,sun2021tree} and prefix disambiguation~\citep{9415054}. These approaches can handle irrelevant and empty contexts but are less scalable when applied to subword units~\citep{pundak2018deep}. Furthermore, a static biasing vocabulary is unsuitable for some applications, including the one described in this paper. Recent works propose hybrid systems to apply both shallow and deep fusion based biasing to achieve state-of-the-art results~\citep{le2021contextualized}. Spelling correction models are also included for additional accuracy gains~\citep{wang2021light,leng2021fastcorrect}. 
%\cite{li2021improving,muralidharan2021noise,mcdermott2019density,prabhavalkar2021less,sun2021tree,le2021contextualized}
